The Rise-Contact involution on Tamari intervals

We describe an involution on Tamari intervals and m-Tamari intervals. This involution switches two sets of statistics known as the "rises" and the "contacts" and so proves an open conjecture from Pr\'eville-Ratelle on intervals of the m-Tamari lattice.

==> figures/decomp-interval-posets/I1.tex <==

\begin{tikzpicture}[scale=.8]
\node(T1) at (0,0) {1};
\end{tikzpicture}

==> figures/decomp-interval-posets/v2.tex <==

\begin{tikzpicture}[scale=1]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (1,-1) {3};
\draw[line width = 2, color=red] (T3) -- (T2);
\draw[line width = 0.5, color=blue] (T1) -- (T2);
\end{tikzpicture}

==> figures/decomp-interval-posets/v4.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013

\begin{tikzpicture}[scale=0.9]
\node(T1) at (0,0) {1};
\node(T3) at (1,-1) {3};
\node(T2) at (1,0) {2};
\node(T4) at (3,0) {4};
\node(T5) at (2,-1) {5};
\node(T6) at (3,-1) {6};
\node(T7) at (4,-1) {7};
\node(T8) at (4,-2) {8};
\draw[line width = 0.5, color=blue] (T1) -- (T2);
\draw[line width = 0.5, color=blue] (T2) -- (T4);
\draw[line width = 0.5, color=blue] (T3) -- (T4);
\draw[line width = 0.5, color=red] (T3) -- (T2);
\draw[line width = 0.5, color=blue] (T6) -- (T7);
\draw[line width = 0.5, color=red] (T8) -- (T7);
\draw[line width = 2, color=red] (T5) -- (T4);
\draw[line width = 2, color=red] (T6) -- (T4);
\end{tikzpicture}

==> figures/decomp-interval-posets/v5.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013

\begin{tikzpicture}[scale=1]
\node(T1) at (-1,-1) {1};
\node(T2) at (0,-1) {2};
\node(T3) at (1,-1) {3};
\node(T4) at (1,-2) {4};
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=red] (T4) -- (T3);
\end{tikzpicture}


==> figures/decomp-interval-posets/v7.tex <==

\begin{tikzpicture}[scale=1]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (1,-1) {3};
\draw[line width = 2, color=red] (T3) -- (T2);
\draw[line width = 0.5, color=blue] (T1) -- (T2);
\end{tikzpicture}

==> figures/interval-posets/I1.tex <==

\begin{tikzpicture}[scale=.8]
\node(T1) at (0,0) {1};
\end{tikzpicture}

==> figures/interval-posets/I2-ex1.tex <==
% Auteur : Viviane Pons
% Création : 16/05/2013


\begin{tikzpicture}[scale=0.8]
\node(T1) at (0,0) {1};
\node(T2) at (0,-1) {2};
\draw[line width = 0.5, color=red] (T2) -- (T1);
\end{tikzpicture}



==> figures/interval-posets/I3-ex3.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013


\begin{tikzpicture}[scale=1]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (1,-1) {3};
\draw[line width = 0.5, color=blue] (T1) -- (T2);
\draw[line width = 0.5, color=red] (T3) -- (T2);
\end{tikzpicture}


==> figures/interval-posets/I3-ex4.tex <==
% Auteur : Viviane Pons
% Création : 16/05/2013

\def \wlev{0.5}
\def \hlev{0.8}

\begin{tikzpicture}

\node(N1) at (0,\hlev) {1};
\green{
\node(T1) at (0,0) {2};
\node(T2) at (0,-1) {3};
\draw[line width = 0.5, color=red] (T2) -- (T1);
}
\end{tikzpicture}


==> figures/interval-posets/I3-ex5.tex <==
% Auteur : Viviane Pons
% Création : 16/05/2013

\def \wlev{0.5}
\def \hlev{0.8}

\begin{tikzpicture}

\node(N1) at (0,\hlev) {1};
\green{
\node(T1) at (0,0) {2};
\node(T2) at (0,-1) {3};
\draw[line width = 0.5, color=red] (T2) -- (T1);
}
\draw[line width = 0.5, color=red](T1) -- (N1);
\end{tikzpicture}


==> figures/interval-posets/I3-ex6.tex <==

\begin{tikzpicture}[scale=1]
\node(T1) at (0,0) {1};
\node(T2) at (1,0) {2};
\node(T3) at (1,-1) {3};
\draw[line width = 0.5, color=red] (T3) -- (T2);
\draw[line width = 0.5, color=blue] (T1) -- (T2);
\end{tikzpicture}

==> figures/interval-posets/I4-ex1.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013

\begin{tikzpicture}[scale=1]
\node(T1) at (-1,-1) {1};
\node(T2) at (0,-1) {2};
\node(T3) at (1,-1) {3};
\node(T4) at (1,-2) {4};
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=red] (T4) -- (T3);
\end{tikzpicture}


==> figures/interval-posets/I4-ex2.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013

\def \wlev{0.5}
\def \hlev{0.8}

\begin{tikzpicture}[scale=0.8]
\node(T2) at (0,-1) {2};
\node(T1) at (0,0) {1};
\node(T3) at (1,-1) {3};
\node(T4) at (1,-2) {4};
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=red] (T2) -- (T1);
\draw[line width = 0.5, color=red] (T4) -- (T3);
\end{tikzpicture}



==> figures/interval-posets/I4-ex3.tex <==


\begin{tikzpicture}[scale=.8]
\node(T1) at (0,0) {1};
\node(T2) at (0,-1) {2};
\node(T3) at (0,-2) {3};
\node(T4) at (1,-2) {4};
\draw[line width = 0.5, color=red] (T3) -- (T2);
\draw[line width = 0.5, color=red] (T2) -- (T1);
\draw[line width = 0.5, color=blue] (T3) -- (T4);
\end{tikzpicture}

==> figures/interval-posets/I6-ex1.tex <==
% Auteur : Viviane Pons
% Création : 10/05/2013
\def \hlev{0.8}
\def \wlev{0.6}

\begin{tikzpicture}
\node(N1) at (0,0) {1};
\node(N2) at (0.5 * \wlev,-1 * \hlev) {2};
\node(N3) at (\wlev,0) {3};
\node(N4) at (2 * \wlev,0) {4};
\node(N5) at (3 * \wlev,0) {5};
\node(N6) at (3 * \wlev,-1 * \hlev) {6};
\draw (N2) -- (N3);
\draw (N2) -- (N1);
\draw (N6) -- (N5);
\end{tikzpicture}


==> figures/interval-posets/I6-ex6.tex <==


\begin{tikzpicture}[scale=1]
\node(T1) at (0,0) {1};
\node(T2) at (0,-1) {2};
\node(T3) at (1,0) {3};
\node(T4) at (2,0) {4};
\node(T5) at (1,-1) {5};
\node(T6) at (2,-1) {6};
\draw[line width = 0.5, color=blue] (T1) -- (T3);
\draw[line width = 0.5, color=blue] (T2) -- (T3);
\draw[line width = 0.5, color=blue] (T3) -- (T4);
\draw[line width = 0.5, color=blue] (T5) -- (T6);
\end{tikzpicture}

==> figures/trees/T2-1.tex <==
% Auteur : Viviane Pons

%       .
%     ./

\begin{tikzpicture}
\node (N0) at (1.250, 0.000){};
\node (N00) at (0.750, -0.500){};
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/trees/T2-2.tex <==
% Auteur : Viviane Pons

%       .
%        \.

\begin{tikzpicture}
\node (N0) at (0.250, 0.000){};
\node (N01) at (0.750, -0.500){};
\draw[Point] (N01) circle;
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/trees/T3-1-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%   ./

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T3-1.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./
%   ./

\begin{tikzpicture}
\node (N0) at (1.250, 0.000){};
\node (N00) at (0.750, -0.500){};
\node (N000) at (0.250, -1.000){};
\draw[Point] (N000) circle;
\draw (N00.center) -- (N000.center);
\draw[Point] (N00) circle;
\draw (N0.center) -- (N00.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/trees/T3-2-n.tex <==
% Auteur : Viviane Pons
% Création 27/04/2013

%       .
%     ./
%      \.

\begin{tikzpicture}
\node (N0) at (2.500, 0.000){3};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T3-3-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%       ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N010) at (1.500, -2.000){2};
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T3-3.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%       ./

\begin{tikzpicture}
\node (N0) at (0.250, 0.000){};
\node (N01) at (1.250, -0.500){};
\node (N010) at (0.750, -1.000){};
\draw[Point] (N010) circle;
\draw (N01.center) -- (N010.center);
\draw[Point] (N01) circle;
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/trees/T3-4-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%       .
%     ./ \.
%       

\begin{tikzpicture}[scale=0.8]
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (2.500, -1.000){3};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T3-4.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%     ./ \.
%       

\begin{tikzpicture}
\node (N0) at (0.750, 0.000){};
\node (N00) at (0.250, -0.500){};
\draw[Point] (N00) circle;
\node (N01) at (1.250, -0.500){};
\draw[Point] (N01) circle;
\draw (N0.center) -- (N00.center);
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/trees/T3-5-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%       .
%        \.
%          \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (2.500, -2.000){3};
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T3-5.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%       .
%        \.
%          \.

\begin{tikzpicture}
\node (N0) at (0.250, 0.000){};
\node (N01) at (0.750, -0.500){};
\node (N011) at (1.250, -1.000){};
\draw[Point] (N011) circle;
\draw (N01.center) -- (N011.center);
\draw[Point] (N01) circle;
\draw (N0.center) -- (N01.center);
\draw[Point] (N0) circle;
\end{tikzpicture}

==> figures/trees/T4-1-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%      /
%     /
%    /

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (2.500, -1.000){3};
\node (N000) at (1.500, -2.000){2};
\node (N0000) at (0.500, -3.000){1};
\draw (N000) -- (N0000);
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-10-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%        ./
%      ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (2.500, -2.000){3};
\node (N0100) at (1.500, -3.000){2};
\draw (N010) -- (N0100);
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-11-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%        ./
%         \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (1.500, -2.000){2};
\node (N0101) at (2.500, -3.000){3};
\draw (N010) -- (N0101);
\draw (N01) -- (N010);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-12-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%         \.
%        ./ \.
%        

\begin{tikzpicture}[scale=0.8]
\node (N0) at (0.500, 0.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N010) at (1.500, -2.000){2};
\node (N011) at (3.500, -2.000){4};
\draw (N01) -- (N010);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-13-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%         \.
%           \.
%          ./

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (3.500, -2.000){4};
\node (N0110) at (2.500, -3.000){3};
\draw (N011) -- (N0110);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-14-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%         \.
%           \.
%             \.

\begin{tikzpicture}
\node (N0) at (0.500, 0.000){1};
\node (N01) at (1.500, -1.000){2};
\node (N011) at (2.500, -2.000){3};
\node (N0111) at (3.500, -3.000){4};
\draw (N011) -- (N0111);
\draw (N01) -- (N011);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-2-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%    ./
%     \

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (2.500, -1.000){3};
\node (N000) at (0.500, -2.000){1};
\node (N0001) at (1.500, -3.000){2};
\draw (N000) -- (N0001);
\draw (N00) -- (N000);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-3-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%    ./\.

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\node (N001) at (2.500, -2.000){3};
\draw (N00) -- (N000);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-4-n.tex <==
% Auteur : Viviane Pons
% Création 26/04/2013

%        .
%      ./
%       \.
%      ./

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (2.500, -2.000){3};
\node (N0010) at (1.500, -3.000){2};
\draw (N001) -- (N0010);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-5-n.tex <==
% Auteur : Viviane Pons
% Création 28/04/2013

%        .
%      ./
%       \.
%        \.

\begin{tikzpicture}
\node (N0) at (3.500, 0.000){4};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\node (N0011) at (2.500, -3.000){3};
\draw (N001) -- (N0011);
\draw (N00) -- (N001);
\draw (N0) -- (N00);
\end{tikzpicture}

==> figures/trees/T4-6-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%     ./

\begin{tikzpicture}[scale=0.8]
\node (N0) at (2.500, 0.000){3};
\node (N00) at (1.500, -1.000){2};
\node (N000) at (0.500, -2.000){1};
\draw (N00) -- (N000);
\node (N01) at (3.500, -1.000){4};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-7-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%       \.

\begin{tikzpicture}[scale=0.7]
\node (N0) at (2.500, 0.000){3};
\node (N00) at (0.500, -1.000){1};
\node (N001) at (1.500, -2.000){2};
\draw (N00) -- (N001);
\node (N01) at (3.500, -1.000){4};
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-8-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%        ./

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (3.500, -1.000){4};
\node (N010) at (2.500, -2.000){3};
\draw (N01) -- (N010);
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}

==> figures/trees/T4-9-n.tex <==
% Auteur : Viviane Pons
% Création 29/04/2013

%        .
%      ./ \.
%           \.

\begin{tikzpicture}
\node (N0) at (1.500, 0.000){2};
\node (N00) at (0.500, -1.000){1};
\node (N01) at (2.500, -1.000){3};
\node (N011) at (3.500, -2.000){4};
\draw (N01) -- (N011);
\draw (N0) -- (N00);
\draw (N0) -- (N01);
\end{tikzpicture}
